Weitzman's Rule for Pandora's Box with Correlations

Pandora's Box is a central problem in decision making under uncertainty that can model various real life scenarios. In this problem we are given $n$ boxes, each with a fixed opening cost, and an unknown value drawn from a known distribution, only revealed if we pay the opening cost. Our goal is to find a strategy for opening boxes to minimize the sum of the value selected and the opening cost paid. In this work we revisit Pandora's Box when the value distributions are correlated, first studied in Chawla et al. (arXiv:1911.01632). We show that the optimal algorithm for the independent case, given by Weitzman's rule, directly works for the correlated case. In fact, our algorithm results in significantly improved approximation guarantees compared to the previous work, while also being substantially simpler. We finally show how to implement the rule given only sample access to the correlated distribution of values. Specifically, we find that a number of samples that is polynomial in the number of boxes is sufficient for the algorithm to work.

==> one_vs_pa_old.tex <==
We begin by showing how Weitzman's algorithm can be extended to correlated distributions. Our algorithm calculates a reservation value $\s$ for every box at each step, and opens the box $b\in \boxes$ with the minimum $\s_b$. We stop if the value is less than the reservation value calculated, and proceed in making this box \emph{free}; we can re-open this for no cost, to obtain the value just realized at any later point. The formal statement is shown in Algorithm~\ref{alg:weitzman_main}. This algorithm obtains an almost tight constant factor approximation, as stated in Theorem~\ref{thm:main_vs_pa}.\\

% As in the original algorithm~\cite{Weit1979}, we stop whenever the best value so far is better than the next reservation value. 

% The key difference in this algorithm, is that we keep track of the \emph{feasible} scenarios at each time step. We call a scenario $s\in \scenarios$ \emph{feasible} at time $t$ if after opening $t-1$ boxes, the values found so far exist in the support of $s$, i.e. this scenario \textbf{can} happen. Denote by $R_t$ the set of feasible scenarios at time $t$; we calculate the reservation value of box $b\in \boxes$ as follows
%


% \evagerg{Uncomment here for "generalizing to $c_i\in \mathbb{R}$" section--probably won't need this section at all}
% \input{general_c}

\begin{algorithm}[H]
		\KwIn{Boxes with costs $c_i\in \mathbb{R}$, distribution over scenarios $\mathcal{D}$.}
        %\ForEach{time step $t$}{
        An unknown vector of values $v \sim \mathcal{D}$ is drawn\\
        
        \Repeat{termination}{
        Calculate $\sigma_b$ for each box $b \in \boxes$\\
        Open box $b = \text{argmin}_{b\in \boxes}\sigma_b$ and stop if the value the observed $V_b = v_b \le \sigma_b$\\
        $c_b\leftarrow 0$ \tcp{This box is open from now on}
        Update the prior distribution
        \begin{itemize}
            \item[-] \textbf{Variant 1}: $\mathcal{D} \leftarrow \mathcal{D}|_{V_b > \sigma_b}$
            \item[-] \textbf{Variant 2}: $\mathcal{D} \leftarrow \mathcal{D}|_{V_b = v_b} $
        \end{itemize}}	
		\caption{Weitzman's algorithm, for correlated distributions. }\label{alg:weitzman_main}
	\end{algorithm}

% \todo{discuss a bit structure:
% \begin{enumerate}
%     \item Strusture 1: 
%     \begin{enumerate}
%         \item 3: main algo with both variants, Thm says both variants get approx factor + discuss LB (applies to all)
%         \item 3.2 proof/discussion of var 1
%         \item 3.2 proof/discussion of var 2
%         \item 4: learnability, why variant 2 isn't learnable, thm 4.1 says var 1 is learnable. show proof
%         \end{enumerate}
%     \item Strusture 2: 
%         \begin{enumerate}
%         \item 3: only talk about variant $v>\sigma$ main algo, Thm gives approx factor for variant + LB. Lemma with LB from MSSC
%         \item 3.1 proof of factor
%         \item 3.2 learnability of this variant, thm says it;s learnable + proof
%         \item 4: variant $V=v$, theorem for approx factor
%         \item 4.1 proof sketch for approx factor
%         \item 4.2 Lernability discussion, this variant isn't learnable + include examples
%         \end{enumerate}
% \end{enumerate}
% }

% \begin{algorithm}[H]%%%OLD VERSION
% 		\KwIn{Boxes with costs $c_i\in \mathbb{R}$, set of scenarios $\scenarios$.}
%         $\mathcal{O} = \emptyset$ \tcp{set of opened boxes}
%         $R_0 \leftarrow \scenarios$ \tcp{Set of feasible scenarios}
%         \ForEach{time step $t$}{
%         Calculate $\sigma_i$ for each box $i\in \boxes$\\
%         Open $b = \text{argmin}_{i\in \boxes}\sigma_i$\\

%         \If{$\min_{b\in \mathcal{O}} v_b \leq   \min_{i\in \boxes \setminus\{b\}} \sigma_{i}$}{
%             Stop\\
%         }
%         $\mathcal{O} \leftarrow \mathcal{O} \cup \{b\}$\\
%         $c_b\leftarrow 0$ \tcp{This box is open from now on}
%         $R_{t+1} \leftarrow R_t \setminus $ {infeasible scenarios}
%         }	
% 		\caption{Weitzman's algorithm, for correlated distributions. }\label{alg:weitzman_main}
% 	\end{algorithm}


\begin{restatable}{theorem}{mainThm}\label{thm:main_vs_pa}
	Algorithm~\ref{alg:weitzman_main} is a $4.428$-approximation for \pbText{}
  %$3+2\sqrt{2} \approx 5.828$-approximation 
  % for $\pb$ when $v_b^s, c_b\in \mathbb{R}$, 
  against the partially-adaptive optimal.
  % , when conditioning on $V_b > \sigma_b$.
\end{restatable}



\todo{check notation in the end to have b for boxes instead of i}


Observe that for independent distributions this algorithm is exactly the same as Weitzman's \cite{Weit1979}, since the product prior $\dist$ remains the same, regardless of the values realized. Therefore, the calculation of the reservation values does not change in every round, and suffices to calculate them only once at the beginning.



\paragraph{Scenarios} To proceed with the analysis of Theorem~\ref{thm:main_vs_pa}, we assume that $\dist$ is supported on a collection of $m$ vectors, $(\vec v^s)_{s \in \scenarios}$, which we call scenarios, and sometimes abuse notation to say that a scenario is sampled from the distribution $\dist$. 
We assume that all scenarios have equal probability. The general case with unequal probabilities follows by creating more copies of the higher probability scenarios until the distribution is uniform.


A scenario is \emph{covered} when the algorithm decides to stop and choose a value from the opened boxes. For a specific scenario $s\in\scenarios$ we denote by $c(s)$ the total opening cost paid by an algorithm before this scenario is covered and by $v(s)$ the value chosen for this scenario.


% Recall that in the independent distribution case the reservation value $\s_b \in \mathbb{R}_+$ for box $b\in \boxes$ is defined as the value $\s$ that satisfies
% \[\E{v\sim \mathcal{D}_b}{(\s-v)^+} = c_b.\]


%
\paragraph{Reservation Values}
% \todo{show equivalent definition}
To analyze Theorem~\ref{thm:main_vs_pa}, we introduce a new way of defining the reservation values of the boxes that is equivalent to~\eqref{eq:reservation_value}.
For a box $b$, we have that

\[\s_b = \min_{A \subseteq \scenarios} \frac{c_b+ \sum_{s\in A} \Pr{\dist}{s} v^s_b}{\sum_{s\in A} \Pr{\dist}{s}} \]

The equivalence to~\eqref{eq:reservation_value}, follows since $\s_b$ is defined as the root of the expression
\begin{align*}
      \E{s \sim \mathcal{D}}{(\s_b-v^s_b)^+} - c_b = \sum_{s\in \scenarios} \Pr{\dist}{s} (\s_b - v^s_b)^+ - c_b = \max_{A \subseteq \scenarios} \sum_{s\in A} \Pr{\dist}{s} (\s_b - v^s_b)  - c_b.
\end{align*}

Thus, $\s_b$ is also the root of
\begin{align*}
      \max_{A \subseteq \scenarios} \frac { \sum_{s\in A} \Pr{\dist}{s} (\s_b - v^s_b)  - c_b } {\sum_{s\in A} \Pr{\dist}{s}} = \s_b - \min_{A \subseteq \scenarios} \frac { c_b + \sum_{s\in A} \Pr{\dist}{s} v^s_b } {\sum_{s\in A} \Pr{\dist}{s}}.
\end{align*}


% For any box $b\in \boxes$ with reservation value $\s_b$ and value $V_b$, denote by $A\subseteq \scenarios$ the points in the support $v\in \mathcal{D}$ for which $\s_b \geq v$. Then we rewrite Equation~\eqref{eq:reservation_value} as
% $c_b = \sum_{s\in A} \Pr{\dist}{s}(\s_b- v_b^s) $ or equivalently
% %
% \[\s_b = \frac{c_b+ \sum_{s\in A} \Pr{\dist}{s} v_b^s}{\sum_{s\in A} \Pr{\dist}{s}}\]

This, gives our formula for computing $\s_b$, which we can further simplify using our assumption that all scenarios have equal probability. In this case, $ \Pr{\dist}{s}= 1/|\scenarios|$ which implies that
%
\begin{equation}\label{eq:equivalent_reserv}
\s_b = \min_{A \subseteq \scenarios} \frac{c_b|\scenarios|+\sum_{s\in A}v_s}{|A|}.
\end{equation}


\subsection{Conditioning on $V_b>\sigma_b$}\label{subsec:proof_algo}

We start by describing the simpler variant of our algorithm where after opening each box we update the distribution by conditioning on the event $V_b > \s_b$. This algorithm is \emph{partially adaptive}, since the order for each scenario does not depend on the actual value that is realized every time. At every step the algorithm will either stop or continue opening boxes conditioned on the event ``We have not stopped yet" which does not differentiate among the surviving scenarios.

\begin{restatable}{theorem}{mainThm}\label{thm:main_vs_pa}
Algorithm~\ref{alg:weitzman_main} is a $4.428$-approximation  
  for \pbText{} 
  % when $v_{ij}, c_i\in \mathbb{R}$,
  against the partially-adaptive optimal, when conditioning on $V_b > \sigma_b$.
\end{restatable}

In this section we show a simpler proof for Theorem~\ref{thm:main_vs_pa} that gives a $3+2\sqrt{2} \approx 5.828$-approximation. The full proof for the $4.428$-approximation is given in section~\ref{apn:main_algo} of the Appendix. Using the equivalent definition of the reservation value (Equation~\eqref{eq:equivalent_reserv}) we can rewrite Algorithm~\ref{alg:weitzman_main} as follows.\\

\begin{algorithm}[H]
				\KwIn{Boxes with costs $c_i\in \mathbb{R}$, set of scenarios $\scenarios$.}
            $t\leftarrow 0$\\
		$R_0 \leftarrow \mathcal{S}$ the set of scenarios still uncovered\\
			\While{$R_t\neq \emptyset$}{
				Let $\s_t \leftarrow \text{min}_{b\in \boxes, A\subseteq R_t} \frac{c_b|R_t| + \sum_{s\in A}v^s_{b}}{|A|}$\\
      Let $b_t$ and $A_t$ be the box and the set of scenarios that achieve the minimum\\
				Open box $b_t$ and pay $c_{b_t}$\\
    Stop and choose the value at box $b_t$ if it is less than $\s_t$: this holds \textbf{iff} $s \in A_t$\\
                Set $c_{b_t} \leftarrow 0$\\
				$R_t \leftarrow R_t \setminus A_t$\\
				$t\leftarrow t+1$
		}
			\caption{Greedy algorithm    }\label{alg:general_v}
	\end{algorithm}
 

\todo{add a line figure for structure of solution}

We first start by giving a bound on the cost of the algorithm. 
The cost can be broken down into opening cost plus the value obtained. 
Since at any time $t$, all remaining scenarios $R_t$ pay the opening cost $c_{b_t}$, we have that the total opening cost is $$\sum_t c_{b_t} |R_t|.$$ Moreover,
the chosen value is given as $$\sum_t \sum_{s \in A_t} v^s_{b_t}. $$
Overall, we have that
$$\alg = \sum_t \left( c_{b_t} |R_t| + \sum_{s \in A_t} v^s_{b_t} \right) = \sum_t |A_t| \frac {  c_{b_t} |R_t| + \sum_{s \in A_t} v^s_{b_t} } { |A_t|} = \sum_t |A_t| \s_t. $$
Defining $\s_s$ to be the reservation value of scenario $s$ at the time it is covered, i.e. when $s \in A_t$, we get $\alg = \sum_{s \in \scenarios} \s_s$.

We follow a \emph{histogram analysis} similar to the proof of Theorem~4 in \cite{FeigUrieLovaTeta2004} for \msscText{} and construct the following histograms.
\begin{itemize}
	\item The $\opt_o$ histogram: put the scenarios on the x-axis on increasing
opening cost order $c_s^\opt$ according to $\opt$, the height of each scenario is the opening cost it paid. 
	\item The $\opt_v$ histogram: put the scenarios on the x-axis on increasing
covering value order $v_s^\opt$ according to $\opt$, the height of each scenario is the value with which it
was covered.
	\item The $\alg$ histogram: put scenarios on the x-axis in the order the algorithm covers them. The height of each scenario is $\s_s$. Observe that the area of the $\alg$ histogram is exactly the cost of the algorithm.
 % For each scenario $s\in \scenarios$ we assign a reservation value $\s_s$ which corresponds to the $\s$ at the step the algorithm covered this scenario, this is the height of each $s$ in the histogram.
 % put scenarios on the x-axis in the order the algorithm covers them, the height of each scenario is the reservation value $\sigma$ at the time the algorithm covers it.
\end{itemize}

% Consider any point $p$ in the $\alg$ histogram, and let $s$ be its corresponding scenario and $t$ be the time this scenario is covered. 
% % For any point $p$ in the $\alg$ histogram we denote by $R_p$ the set of scenarios uncovered at $p$. Then using the definition of the reservation value we have that
% %
% % \begin{equation}\label{eq:sigma_p}
% % 	\sigma_t = \min_{b\in \boxes, A\subseteq R_p} \frac{c_b|R_p| + \sum_{s\in A}v^s_{b}}{|A|} 
% % 		\leq \frac{c_b|R_p| + \sum_{s\in A}v^s_{b}}{|A|}
% % \end{equation}
% \begin{equation}\label{eq:sigma_p}
% 	\sigma_s = \frac{c_b|R_t| + \sum_{s\in A_t}v^s_{b}}{|A_t|} 
% 		\leq \frac{c_b|R_t| + \sum_{s\in A}v^s_{b}}{|A|}
% \end{equation}
% where the last inequality holds for all $A\subseteq R_t$ and any $b\in \boxes$.


\input{one_pa_optimized}


